LTLf Best-Effort Synthesis in Nondeterministic Planning Domains

We study best-effort strategies (aka plans) in fully observable nondeterministic domains (FOND) for goals expressed in Linear Temporal Logic on Finite Traces (LTLf). The notion of best-effort strategy has been introduced to also deal with the scenario when no agent strategy exists that fulfills the goal against every possible nondeterministic environment reaction. Such strategies fulfill the goal if possible, and do their best to do so otherwise. We present a game-theoretic technique for synthesizing best-effort strategies that exploit the specificity of nondeterministic planning domains. We formally show its correctness and demonstrate its effectiveness experimentally, exhibiting a much greater scalability with respect to a direct best-effort synthesis approach based on re-expressing the planning domain as generic environment specifications.

==> sections/4-best-effort.tex <==
\section{Best-Effort Synthesis in Planning Domains~\label{sec:4}}

In this section, we introduce the problem of \LTLf best-effort synthesis in nondeterministic planning domains. In doing so, we first define what it means for an agent to make a best-effort to achieve a goal. We observe that our definitions adapt those in \cite{ADR2021} to environments represented as planning domains. First, we introduce the notion of dominance of agent strategies,  

% A best-effort strategy is one which guarantees that the agent does its best to achieve a goal without doing anything that unecessarily prevents the goal from being reached. 
% We now formalize the concept of an agent making its best-effort to achieve a goal specified in an \LTLf formula $\varphi$ in a nondeterministic planning domain $\D$. To that end, we start with introducing the dominance of agent strategies, which intuitively corresponds to the amount of efforts that a strategy $\sigma$ indicates.
% We base our definition on the notion of dominance introduced below.
% We specify below what it means for an agent strategy to make a best-effort to achieve a goal on a planning domain. We base our definition on the notion of dominance, which we introduce below.

\begin{definition}~\label{dfn:dominance}
Let \(\D\) be a planning domain, \(\varphi\) an \LTLf goal, and \(\sigma_1\) and \(\sigma_2\) two legal agent strategies, \(\sigma_1\) \textit{dominates} \(\sigma_2\) for \(\varphi\) in \(\D\), written \(\sigma_1 \geq_{\varphi|\D} \sigma_2\), if for every legal environment strategy \(\gamma\), \(\mathtt{Play}(\sigma_2, \gamma) \models_{\D} \varphi\) implies \(\mathtt{Play}(\sigma_1, \gamma) \models_{\D }\varphi\).
\end{definition}

Furthermore, a legal agent strategy \(\sigma_{1}\) \textit{strictly dominates} legal agent strategy \(\sigma_{2}\) for goal \(\varphi\) in \(\D\), written \(\sigma_1 >_{\varphi|\D} \sigma_2\), if \(\sigma_1 \geq_{\varphi|\D} \sigma_2\) and \(\sigma_2 \not \geq_{\varphi|\D} \sigma_1\). Intuitively, \(\sigma_1 >_{\varphi|\D} \sigma_2\) shows that \(\sigma_1\) does at least as well as \(\sigma_2\) against every legal environment strategy in \(\D\) and strictly better against at least one such strategy. If $\sigma_1$ strictly dominates $\sigma_2$, then an agent using $\sigma_2$ is not doing its “best” to achieve the goal.
% In particular, if \(\sigma_2\) is not maximal, say \(\sigma_1\) strictly dominates it, then an agent that uses $\sigma_2$ is not doing its “best” to achieve the goal. 
% if it used $\sigma_2$ instead, it could achieve the goal against a strictly larger set of environment reactions.
Within this framework, a best-effort solution is one that is not strictly dominated by any other strategy.

\begin{definition}~\label{dfn:best-effort}
A legal agent strategy $\sigma$ is a best-effort solution for $\varphi$ in $\D$ iff there is no legal agent strategy $\sigma'$ such that $\sigma' >_{\varphi|\D} \sigma$.
\end{definition}

Observe that differently from~\cite{ADR2021}, in our framework best-effort solutions are also required to be legal, i.e., to always respect agent action preconditions. Indeed, the agent has no such preconditions to follow when the environment is specified as an \LTL/\LTLf formula. Furthermore, the following is immediate from Definition~\ref{dfn:best-effort}.

\begin{proposition}
Let $\D$ be a planning and $\varphi$ an \LTLf goal that admits a strong solution in $\D$. Then, $\sigma$ is a best-effort solution for $\varphi$ in $\D$ iff $\sigma$ is a strong solution for $\varphi$ in $\D$.
\end{proposition}

Alternatively to Definition~\ref{dfn:best-effort}, we can characterize best-effort solutions locally using the notion of value of a history wrt an agent goal $\varphi$ and a planning domain $\D$. Intuitively, a history $h$ can be assigned a value specifying whether the agent can extend $h$ and win, lose, or neither. With this notion, we can characterize a best-effort solution $\sigma$ as maximizing the value of every history $h$ consistent with it.

Formally, a history is a finite and legal sequence of states of a planning domain $\D$. For a history $h$ and a legal agent strategy $\sigma$, we use $\Gamma(h, \sigma)$ to denote the set of legal environment strategies $\gamma$ in $\D$  such that $h$ is a proper prefix of $\Play(\sigma, \gamma)$. Furthermore, we denote by $\H(\sigma)$ the set of legal histories $h$ such that $\Gamma(h, \sigma)$ is nonempty, i.e., the set of legal histories of $\D$ consistent with $\sigma$ for some environment strategy $\gamma$. Next, we define:

\begin{compactitem}
    \item $\val(\sigma, h) = +1$ (winning), if $\Play(\sigma, \gamma) \pmodels \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    \item $\val(\sigma, h) = -1$ (losing), if $\Play(\sigma, \gamma) \not \pmodels \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    \item $\val(\sigma, h) = 0$ (pending), otherwise.
\end{compactitem}

Let $\val(h)$ be the maximal value of $\val(\sigma, h)$, considering all the strategies $\sigma$ such that $h \in \H_{\D}(\sigma)$\footnote{We consider $\val(h)$ only if there exists at least one agent strategy $\sigma$ such that $h \in \H_{\D}(\sigma)$.}. The following theorem follows from the above characterization.
% The following theorem states that we can characterize a best-effort strategy $\sigma$ with the maximal value 

\begin{theorem} [Maximality Condition]\label{thm:max}
A legal agent strategy $\sigma$ is a best-effort solution for $\varphi$ in $\D$ iff for each $h \in \H_{\D}(\sigma)$ it holds that $\val_{\varphi|\D}(\sigma, h) = \val_{\varphi|\D}(h)$.
\end{theorem}

Intuitively, Theorem~\ref{thm:max} above states that a strategy $\sigma$ is a best-effort solution if, for every history $h$ that is consistent with it, the following properties hold: \myi if the agent can extend $h$ and achieve the goal regardless of environment reactions, then any extension of $h$ following $\sigma$ ensures goal completion; \myii if any extension of $h$ do not allow the agent to achieve the goal, then $\sigma$ just behaves legally; \myiii else, if some extension of $h$, but not all, allows the agent to achieve the goal, then there exists an extension of $h$ following $\sigma$ ensuring goal completion. Observe that in \myiii the agent does its best by assuming that the environment might possibly cooperate, thus helping the agent towards achieving its goal. 

% It should be noted that our definition is similar to that in~\cite{ADR2021}. However, when the environment is specified as a planning domain, best-effort solutions are also required to respect agent action preconditions, i.e., to be legal. Differently, 
% It should be noted the similarity that exists between our notion of dominance and that given by~\cite{ADR2021}. In particular, when the environment is specified as a planning domain, this domain also consists of the preconditions of the agent's actions. Instead, when the environment is specified in an \LTL/\LTLf formula, there are no such preconditions that the agent needs to follow~\cite{ADR2021}. 
% % our definition restricts both environment and agent strategies to those that are legal (vs. those that enforce an \LTLf environment assumption and no restriction, respectively). 

% It is immediate to see from the definition that it holds the following:
% From the definition, it is immediate that for a realizable goal then a legal agent strategy that realizes it is a best-effort strategy. 
% From the definition it trivially holds the following:
% From the definition, it immediately follows:

% \begin{proposition}
% Let $\D$ be a planning domain, $\varphi$ an \LTLf goal realizable on $\D$, and $\sigma$ a legal agent strategy. Then, $\sigma$ realizes $\varphi$ on $\D$ iff $\sigma$ is best-effort for $\varphi$ on $\D$
% \end{proposition}

% Best-effort synthesis is the problem of finding a best-effort strategy for a goal on a planning domain.
\LTLf best-effort synthesis in nondeterministic planning domains concerns computing a best-effort solution for a  goal in some domain. 

\begin{definition}~\label{def:best-effort-synthesis}
The problem of \LTLf best-effort synthesis in nondeterministic planning domains is defined as a pair $\P = (\D, \varphi)$, where $\D$ is a planning domain and $\varphi$ is an \LTLf formula. Best-effort synthesis of $\P$ computes a best-effort solution for $\varphi$ in $\D$.
\end{definition}

While classical synthesis and planning settings (see e.g.~\cite{PR89,DegVa15,DeGR18}) first require checking the realizability of the problem, i.e., the existence of a solution, in the case of best-effort synthesis realizability is trivial, as there always exists a best-effort solution.

% Differently from classical synthesis settings (see e.g.~\cite{PR89,DegVa15}), which first require checking the realizability of the problem, in the case of best-effort synthesis realizability is trivial, as there is always a best-effort solution. \gp \textcolor{red}{Change this sentence to include strong and cooperative solutions}
\begin{theorem}~\label{thm:existence}
Let $\P = (\D, \varphi)$ be a problem of \LTLf best-effort synthesis in nondeterministic planning domains. There exists a best-effort solution $\sigma$ for $\varphi$ in $\D$. 
\end{theorem}

In order to prove Theorem~\ref{thm:existence}, we show that we can always construct a strategy $\sigma^*$ that satisfies the Maximality Condition. To do so, we construct a chain of legal agent strategies $\sigma_0, \sigma_1, \ldots$ by selecting for each $i \geq 0$, a history $h \in \H(\sigma_i)$ that has not yet been marked as stabilized, i.e., $val(\sigma_i, h) < val(h)$, and maximizing the value $val(\sigma_{i+1}, h)$. $\sigma_{i+1}$ is constructed by selecting a strategy $\sigma$ such that $val(\sigma, h) = val(h)$ and setting $\sigma_{i+1} = \sigma_i[h \leftarrow \sigma]$, where $\sigma_i[h \leftarrow \sigma]$ denotes the strategy that agrees with $\sigma_i$ everywhere, except in $h$ and all its extensions where it agrees with $\sigma$. $\sigma^*$ is the point-wise limit of the chain of strategies, i.e., $\sigma^* = lim_{i} \ \sigma_{i}$.\footnote{Full proofs can be found in the supplementary material.}



% Intuitively, we based the proof of Theorem 2 on the construction by~\cite{ADLMR21a}, which shows the existence of a best-effort strategy \LTL goals and environment assumptions.

% Proving this theorem requires an alternative characterization for dominance and best-effort strategies, which we now sketch. We begin by formalizing the main notions.
% 
% First, we denote by $h$ a history of a planning domain, which is a finite and legal sequence of states. For a legal history $h$ and a legal agent strategy $\sigma$, we use $\Gamma(h, \sigma)$ to denote the set of legal environment strategies $\gamma$ such that $h$ is a prefix of $\mathtt{Play}(\sigma, \gamma)$. Furthermore, we denote by $\H(\sigma)$ the set of legal histories $h$ such that $\Gamma(h, \sigma)$ is nonempty, i.e., the set of legal histories of $\D$ consistent with $\sigma$ for some environment strategy $\gamma$.

% We base our proof for Theorem 2 on the notion of value. 
% Intuitively, the value of $h$ is $+1$ when all extensions of $h$ that are legal traces realize the agent goal; the value of $h$ is $-1$ when all extensions of $h$ that are legal traces do not realize the agent goal; the value of $h$ is $0$, otherwise.

% A history $h$ can be associated with a value that specifies whether the agent can extend $h$ to win, lose, or neither. With $h$, we can characterize a best-effort solution $\sigma$ as a strategy that maximizes the value of every history $h$ that is consistent with it. More specifically:
% Now, define: 
% \begin{compactitem}
    % \item $val(\sigma, h) = +1$ (winning), if $\mathtt{Play}(\sigma, \gamma) \models_{\D} \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    % \item $val(\sigma, h) = -1$ (losing), if $\mathtt{Play}(\sigma, \gamma) \not \models_{\D} \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    % \item $val(\sigma, h) = 0$ (pending), otherwise.
% \end{compactitem}

% Let $val(h)$ be the maximal value of $val(\sigma, h)$, considering all the strategies $\sigma$ such that $h \in \H(\sigma)$\footnote{We consider $val(h)$ only if there exists more than one agent strategy $\sigma$ such that $h \in \H(\sigma)$.}. 
% The following theorem states that we can characterize a best-effort strategy $\sigma$ with the maximal value 

% \begin{theorem}
% A legal agent strategy $\sigma$ is best-effort iff for each $h \in \H(\sigma)$ it holds that $val(\sigma, h) = val(h)$.
% \end{theorem}

% Theorem~\ref{thm:max} can be proved by contradiction. In order to prove Theorem~\ref{thm:realizability}, we show that we can always construct a strategy $\sigma^*$ that satisfies the Criterion of Maximality. We start with constructing a chain of legal agent strategies $\sigma_0, \sigma_1, \ldots$ by selecting for each $i \geq 0$, a history $h \in \H(\sigma_i)$ that has not yet been marked as stabilized, i.e., $val(\sigma_i, h) < val(h)$, and maximizing the value $val(\sigma_{i+1}, h)$. $\sigma_{i+1}$ is constructed by selecting a strategy $\sigma$ such that $val(\sigma, h) = val(h)$ and setting $\sigma_{i+1} = \sigma_i[h \leftarrow \sigma]$, where $\sigma_i[h \leftarrow \sigma]$ denotes the strategy that agrees with $\sigma_i$ everywhere, except in $h$ and all its extensions where it agrees with $\sigma$. $\sigma^*$ is the point-wise limit of the chain of strategies, i.e., $\sigma^* = lim_{i} \ \sigma_{i}$.\footnote{Full proofs can be found in the supplementary material.}
% The full proof shows that every history is marked as stabilized at the limit and that $\sigma^*$ satisfies the Criterion of Maximality.

% Intuitively, the Theorem~\ref{thm:max} shows that it is always possible to construct a strategy $\sigma$ that satisfies the Criterion of Maximality, hence being best-effort.


\iffalse

The proof of this theorem requires a sophisticated construction, which we now sketch. We begin by formalizing the main concepts used in the proof.
% Here, we provide formalization of the main concepts used in the proof.

First, we introduce the notion of the value $val(h)$ of a history $h$, that is, a finite, legal sequence of states of the planning domain. Intuitively, the value of $h$ is $+1$ when all extensions of $h$ that are legal traces realize the agent goal; the value of $h$ is $-1$ when all extensions of $h$ that are legal traces do not realize the agent goal; the value of $h$ is $0$, otherwise. With this notion, we can characterize a best-effort strategy as one that maximizes the value of each history that is consistent with it.

For a legal history $h$ and a legal agent strategy $\sigma$, we define $\Gamma(h, \sigma)$ as the set of legal environment strategies $\gamma$, for which $h$ is a prefix of $\mathtt{Play}(\sigma, \gamma)$. Furthermore, we denote by $\H(\sigma)$ the set of histories $h$ such that $\Gamma(h, \sigma)$ is nonempty.

Now, define: \begin{itemize}
    \item $val(\sigma, h) = +1$ (winning) if $\mathtt{Play}(\sigma, \gamma) \models_{\D} \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    \item $val(\sigma, h) = -1$ (losing) if $\mathtt{Play}(\sigma, \gamma) \not \models_{\D} \varphi$ for every $\gamma \in \Gamma(h, \sigma)$;
    \item $val(\sigma, h) = 0$ (pending) otherwise;
\end{itemize}
 
The following Lemma provides an alternative characterization of dominance. 

\begin{lemma}[Characterization of Dominance]
Let $\D$ be a planning domain, $\varphi$ be an \LTLf goal, and $\sigma_1$, $\sigma_2$ be two legal agent strategies. Then: (A) $\sigma_1 \geq_{\varphi|\D} \sigma_2$ iff for every $h \in \H(\sigma_1)$, if $\sigma_1$ and $\sigma_2$ split at $h$ then: \myi $val(\sigma_1, h) \geq val(\sigma_2, h)$ and \myii it is not the case that $val(\sigma_1, h) = val(\sigma_2, h) = 0$. Furthermore, (B) $\sigma_1 >_{\varphi|\D} \sigma_2$ iff \myiii there exists $h \in \H(\sigma_1)$ at which $\sigma_1$ and $\sigma_2$ split such that $val(\sigma_1, h) > val(\sigma_2, h)$.
\end{lemma}

Given legal agent strategies $\sigma_1$, $\sigma_2$ and a legal trace $h$, we denote by $\sigma_1[h \leftarrow \sigma_2]$ the agent strategy that agrees with $\sigma_1$ everywhere, except in $h$ and all its extensions where it agrees with $\sigma_2$. Let $val(h)$ be the maximum value for $val(\sigma, h)$ for any strategy $\sigma$ such that $h \in \H(\sigma)$\footnote{We consider $val(h)$ only in case there exists at least one agent strategy $\sigma$ for which $h \in \H(\sigma)$.}. The following theorem follows from the above characterization.


\begin{theorem} [Criterion of Maximality]
A legal agent strategy $\sigma$ is best-effort iff for each $h \in \H(\sigma)$ it holds $val(\sigma, h) = val(h)$.
\end{theorem}

The proof of Theorem 1 constructs a strategy $\sigma^*$ that satisfies the Criterion of Maximality.

To do this, we construct a chain of legal agent strategies $\sigma_0, \sigma_1, \ldots$ by selecting at each $i \geq 0$, a history $h \in \H(\sigma_i)$ that has not yet been marked as stabilized, i.e., $val(\sigma_i, h) < val(h)$, and maximizing the value $val(\sigma_{i+1}, h)$. $\sigma_{i+1}$ is constructed by selecting a strategy $\sigma$ such that $val(\sigma, h) = val(h)$ and setting $\sigma_{i+1} = \sigma_i[h \leftarrow \sigma]$. $\sigma^*$ is the point-wise limit of the chain of strategies, i.e., $\sigma^* = lim_{i} \ \sigma_{i}$. The full proof shows that every history is marked as stabilized at the limit and that $\sigma^*$ satisfies the Criterion of Maximality.
% and hence is a best-effort strategy.

 % At the limit, every history is marked and $val(\sigma^*, h) = val(h)$ holds for every $h \in \H(\sigma^*)$, hence it follows from the Criterion of maximality that $\sigma^*$ is a best-effort strategy
 
\fi


==> sections/6-correctness.tex <==
\section{Correctness and Complexity}

% This section is devoted to proving the correctness of Algorithm 1 and the complexity of \LTLf best-effort synthesis over planning domains.  

In this section, we prove the correctness of Algorithm 1. In doing so, we compare the games solved in steps 3 and 4 of Algorithm 1 with their corresponding games from the algorithm for \LTLf best-effort synthesis~(both agent goal and environment assumptions are \LTLf formulas) presented in~\cite{ADR2021}. We then establish the complexity of \LTLf best-effort synthesis over nondeterministic planning domains. 

First, consider the \textit{adversarial} game for the agent to satisfy \(\E \supset \varphi\). in ~\cite{AGMR19} it has been proved that solving this game returns an agent strategy to realize the goal $\varphi$ in the environment $\E$. In our setting, the agent 
%wins the game 
realizes $\varphi$ in $\D$ if it never gets to $S^{ag}_{err}$ (i.e., always follow the preconditions of its actions) \textit{and} succeeds in 
% either realizing its goal $\varphi$ or eventually forcing the environment to reach $s^{env}_{err}$ 
% (i.e., forces the environment to violate the preconditions of its reactions). 
reaching $S^{env}_{err} \cup R'_{\varphi}$ (i.e., either force the environment to violate the preconditions for its reactions or succeed in realizing $\varphi$). The first conjunct requires the agent to never visit a state $(s, q)$, where $s = s^{ag}_{err}$, while the second conjunct requires the agent to eventually visit a state \((s, q)\), where $s = s^{env}_{err}$ or $q \in R_{\varphi}$ in order to win. 
In other words, the agent is supposed to enforce the following on $\G$: 
{\centerline{$\Box(\lnot S^{ag}_{err})\land \Diamond(S^{env}_{err}\lor R'_\varphi)$}}
% where $S^{ag}_{err} = \{(s, q) \mid s = s^{ag}_{err}\}$ and $S^{env}_{err} = \{(s, q) \mid s = s^{env}_{err}\}$. 
(For simplicity, we abuse notations and consider sets of states as atomic propositions).
% Here, the agent wins the game if it succeeds in realizing goal \(\varphi\) while never violating the agent action preconditions \textbf{or} eventually having the environment violate its reaction preconditions. 
% Formally, the states of \(\G\) which satisfy these conditions are: 
% $$
% \F_{\D \rightarrow \varphi} = \{(s, q) \mid s \neq s^{ag}_{err} \wedge (s = s^{env}_{err} \vee q \in F_{\varphi})\}.
% $$
%%
For satisfying this condition, we can solve the game $(\G, \safereach(\lnot S^{ag}_{err},\, S^{env}_{err} \cup R'_\varphi))$. The following theorem specifies the relationship between the existence of strategies to realize $\varphi$ in $\D$ and of winning strategies for $(\G, \safereach(\lnot S^{ag}_{err},\, S^{env}_{err} \cup R'_\varphi))$.
% The following theorem holds by construction and specifies the relationship that holds between strategies that realize $\varphi$ on $\D$ and winning strategies for $(\G, SafeReach(\lnot S^{ag}_{err},\, S^{env}_{err}\lor R'_\varphi))$.
% The following theorem specifies the relationship that holds between winning strategies for game $(\G, SafeReach(\lnot S^{ag}_{err},\, S^{env}_{err}\lor \F_\varphi))$ and plans that realize $\varphi$ on $\D$

\begin{theorem}
Let $\D$ be a planning domain and $\varphi$ an \LTLf goal. Then, $\varphi$ has a strong solution in $\D$ iff there exists a winning strategy for $(\G, \safereach(\lnot S^{ag}_{err},\, S^{env}_{err} \cup R'_\varphi))$.
\end{theorem}

% Alternatively, we show that we can equivalently solve the simpler reachability only condition:
Safety-Reachability games can be solved through a reduction to an equivalent reachability game (e.g. see~). In our setting, we can reduce to an even simpler reachability condition:

% \[\Diamond(\lnot S^{ag}_{err}\land (S^{env}_{err}\lor R'_\varphi)),\]
{\centerline{$\Diamond(\lnot S^{ag}_{err}\land (S^{env}_{err}\lor R'_\varphi)).$}}

That is, we just need to solve the \DFA game $(\G, \reach(\lnot S^{ag}_{err}\cap( S^{env}_{err}\cup R'_\varphi)))$, as listed in step 3 of Algorithm 1. The key idea for such reduction is that, due to the specific structure of the domain $\D$, once an error state is reached, the transitions just keep looping there. This allows us to ignore the safety condition and push $\lnot S^{ag}_{err}$ into the reachability condition.

% We define the following winning conditions:
% Safe($T_s$), where $T_s = \{(s, q) \mid s \neq s^{ag}_{err}\}$, and Reach($T_r$), where $T_r = \{(s, q) \mid s = s^{env}_{err} \vee q \in F_{\varphi}\}$. Therefore, in order to achieve $\E \rightarrow \varphi$, the agent is required to force the play to satisfy the condition of Safe($T_s$) $\wedge$ Reach($T_r$). Below, we show that this winning condition can be rewritten with a single reachability condition to the set of states \(T_s \wedge T_r\) 

% In particular, Lemma 2 allows us to rewrite the goal of the adversarial game more simply as $Reach(T_a)$, where \(T_{a} = \{(s, q) \mid s \neq s^{ag}_{err} \wedge (s = s^{env}_{err} \vee q \in F_{\varphi})\} \) 

%Now, we consider the \textit{adversarial} game for the agent on the \textit{negation of the environment} \(\neg \E\) (c.f. step 4 of Algorithm 0). In this case, the agent goal is to force the environment to violate its reaction precondition, thus forcing the play to reach a state $(s, q)$, where \(s = s^{env}_{err}\). Indeed, along the trace to reach such state, the agent needs to always follow its action precondition, i.e., never reaching a state $(s, q)$, where $s = s^{ag}_{err}$. For this game, in symbols, we want the agent to win the following condition on the arena $\G$:
%\[
%\Box(\neg S^{ag}_{err}) \land \Diamond (S_{err}^{env})
%\]
%where $S^{ag}_{err}$ and $S^{env}_{err}$ are defined as above. Indeed, we can also solve it through solving a simpler reachability only condition (as shown in Lemma 2).
%\[
%\Diamond(\neg S^{ag}_{err} \land S_{err}^{env}).
%\]

% that using an argument similar to Lemma 2 we can prove that Safe($T_s$) \(\wedge\) Reach($T^{\neg \D}_r$) is equivalent to Reach($T_s \wedge T^{\neg \D}_r$). In particular, this allows us to rewrite the goal for the negation of the environment as \(Reach(F_{\neg \D})\), where \(F_{\neg \D} = \{(s, q) \ s.t. \ s \neq s^{ag}_{err} \wedge s = s^{env}_{err}\}\) \newline
% \texttt{GP}
% Is it possible to directly write \(F_{\neg \D} = \{(s, q) \ s.t. \ s = s^{env}_{err}\}\)?



%Note that in the current step, we aim to compute the set of agent winning states \(\WinSet_{ag}(\G, SafeReach(\neg S^{ag}_{err}, S_{err}^{env}))\) or, equivalently, \(\WinSet_{ag}(\G, Reach(\neg S^{ag}_{err} \land S_{err}^{env}))\), from where the agent is able to force the winning condition. In fact, we are able to directly collect states in \(\WinSet_{ag}(\G, Reach(\neg S^{ag}_{err} \land S_{err}^{env})\) on the game arena $\G$, without solving the corresponding adversarial game. This derives from the requirement of existence of environment reaction, which make it impossible for the agent to force the environment to violate preconditions for its reactions. 
% except in states where these are already violated. 
% More specifically, the agent winning region for the game \((\G, Reach(\neg S^{ag}_{err} \land S_{err}^{env}))\) coincides precisely with \(\neg S^{ag}_{err} \land S_{err}^{env}\), as stated in the following:

% \begin{lemma}
% Let \(\D\) and \(\varphi\) be a planning domain and an \LTLf agent goal, respectively. Then, \(\WinSet_{ag}(\G, Reach(\neg S^{ag}_{err} \land S_{err}^{env})) = \neg S^{ag}_{err} \land S_{err}^{env}\).
% \end{lemma}

% \begin{proof}

%To prove the lemma, assume by a contradiction that \(\WinSet_{ag}(\G, Reach(\neg S^{ag}_{err} \land S_{err}^{env})) \neq \neg S^{ag}_{err} \land S_{err}^{env}\). Here, we omit the proof for case \(\WinSet_{ag}(\G, Reach(\lnot S^{ag}_{err} \land S_{err}^{env})) \subset S^{ag}_{err} \land S_{err}^{env}\), which is trivial, and consider the case \(\WinSet_{ag}(\G, Reach(\lnot S^{ag}_{err} \land S_{err}^{env})) \supset S^{ag}_{err} \land S_{err}^{env}\), which implies that there exists at least a state \((s, q) \in (2^\F \cup \{s^{ag}_{err}, s^{env}_{err}\}) \times Q\) such that \((s, q) \not \in S^{ag}_{err} \land S_{err}^{env}\) and \((s, q) \in \WinSet_{ag}(\G,  Reach(\lnot S^{ag}_{err} \land S_{err}^{env}))\). It follows from \((s, q) \not \in \lnot S^{ag}_{err} \land S_{err}^{env}\) that either \myi \(s = s^{ag}_{err}\) or \myii \(s \neq s^{env}_{err}\).

% Now, let \((s^*, q^*)\) be such a state. Here, note that if \myi holds, then the agent cannot reach \(\lnot S^{ag}_{err} \land S_{err}^{env}\), since every state \((s^{ag}_{err}, q)\) with \(q \in Q\) is a sink. Now, if \myii holds, then \((s^*, q^*)\) is such that in it the agent can perform an action \(a \in \alpha(s^*) \in \A\), say \(a^*\), such that:
% $$
% \forall r \in \R.\partial((s^*, q^*), (a^*, r)) \in S^{env}_{err}
% $$
% Now, observe that by construction of \(\partial\) from \(\delta'\) then results:
% $$
% \forall r \in \R.\delta'(s^*, a^*, r) = s^{env}_{err}
% $$
% In turn, from the construction of \(\delta'\) we obtain:
% $$
% \forall r \in \R.\delta'(s^*, a^*, r) = s^{env}_{err} \rightarrow a^* \in \alpha(s^*) \wedge r \not \in \beta(s^*, a^*)
% $$
% However, from the environment reaction existence requirement we get:
% $$
% a^* \in \alpha(s^*) \rightarrow \exists r.r \in \beta(s^*, a^*) 
% $$
% That leads to a contradiction and concludes the proof.

% \end{proof}

After solving the game for $\E \supset \varphi$, the algorithm in~\cite{ADR2021} requires solving games for $\neg \E$ and $\E \wedge \varphi$ to compute a strategy to cooperatively realize $\varphi$ in $\E$. In our setting, we do this by solving only one game with a suitable acceptance condition.
% for the agent.
% In our setting, we will prove that we can compute a strategy to cooperatively realize $\varphi$ on $\D$ by solving only one game.
% The algorithm in~\cite{ADR2021} requires solving two games for computing a strategy to cooperatively realize goal $\varphi$ in the environment $\E$: the \textit{adversarial} game for the environment for $\neg \E$ and \textit{cooperative} game for $\E \wedge \varphi$.  

% Now, consider the adversarial game for the \textit{environment} to satisfy $\neg \E$. The algorithm from~\cite{ADR2021} requires solving this game in order to restrict agent and environment behaviors to be cooperative. Then, their algorithm solves the cooperative game $\E \wedge \varphi$ to get a cooperatively winning strategy for goal $\varphi$ in the environment $\E$. 

% Here, consider the adversarial game for the \textit{environment} to satisfy $\neg \E$ and the \textit{cooperative} game for the agent to satisfy $\E \wedge \varphi$. The algorithm in~\cite{ADR2021} requires solving the adversarial game for the environment in order to ensure that the environment cooperates without violating its own specification $\E$ and the second to get a cooperative strategy for the agent to satisfy its goal $\varphi$. 

% Finally, we consider the cooperative game for the agent to satisfy \(\E \wedge \varphi\) (c.f. step 6 of Algorithm 0). 
% In our setting, the agent wins the game for $\E \wedge \varphi$ if it never gets to \(S^{ag}_{err}\) (i.e., never violates preconditions for its actions) \textit{and} if it succeeds in realizing its goal \(\varphi\) while \textit{cooperatively} satisfying the environment specification $\E$. 
% \textit{cooperatively} with the environment. 
% Then, the agent is required 
% Note that in this game the agent is required not to negate the environment specification, i.e., to never get to \(S^{env}_{err}\), where the environment has violated a precondition for its reactions.

% Indeed, if this were the case, the agent would win the adversarial game \((\G, Reach(\lnot S^{ag}_{err} \land S_{err}^{env}))\). 

% Intuitively, the result of Lemma 2 tells us that for no planning domain that satisfies the environment reaction existence requirement the agent can force the environment to violate a precondition for its reactions. Nevertheless, the agent must apply a restriction (c.f. step 5 of Algorithm 0) to prevent that the environment deliberately violates a precondition for its reactions when cooperating (c.f. step 6 of Algorithm 0). However, in the case of planning domains, this restriction is not necessary as we will show below.
% To see this, consider the \textit{cooperative} game for the agent (game for \(\E \wedge \varphi\) on  step 3 of Algorithm 0). 

Observe that the agent cooperatively realizes $\varphi$ in $\D$ if it never visits $S^{ag}_ {err}$ (i.e., it never violates an action precondition) \textit{and} it eventually reaches $R'_ {\varphi}$ (i.e., it succeeds in realizing $\varphi$) \textit{cooperatively} with the environment. Moreover, note that the environment is also required to never visit $S^{env}_{err}$, as doing so would violate reaction preconditions.
% 
% Here, for the environment to be cooperative it is required that it never reaches $S^{env}_ {err}$, as doing so  
% To see this, observe that to cooperatively realize $\varphi$ on $\D$ the agent is required to never violated precondition for its reactions and to eventually satisfy its goal \textit{cooperatively} with the environment. Here, the agent assumes    
% Here, the agent wins the game if it always respects the preconditions for its actions and eventually realizes its goal cooperatively with the environment. In this case, note that the cooperativity of the environment requires that preconditions for environment reactions are not violated, i.e., the agent expects the environment to cooperate without deliberately violating preconditions for its reactions (which incidentally would cause the agent to win in the adversarial game on the negation of the environment).  
% 
The first conjunct describes that the agent never reaches a state \((s, q) \ s.t. \ s \in \{s^{env}_{err}, s^{ag}_{err}\}\), while the second conjunct requires the agent to eventually reach a state \((s, q) \ s.t. \ q \in R'_{\varphi}\) in order to win. In other words, the agent is supposed to enforce the following condition on \(\G\), should the environment \textit{cooperate}:

{\centerline{$\Box(\neg S^{ag}_{err}) \land \Box (\neg S^{env}_{err}) \land \Diamond (R'_{\varphi}).$}}

In order to do so, we can solve the game $(\G, \safereach(\lnot S^{ag}_{err} \cap \lnot S^{env}_{err}. R'_{\varphi}))$, considering the environment being \textit{cooperative}. The following theorem specifies the relationship between the existence of strategies to \textit{cooperatively} realize $\varphi$ in $\D$ and of \textit{cooperatively} winning strategies for $(\G, \safereach(\lnot S^{ag}_{err} \cap \lnot S^{env}_{err}, R'_\varphi))$.

% The following theorem holds by construction and specifies the relationship that holds between strategies that cooperatively realizes $\varphi$ on $\D$ and cooperatively winning strategies on $(\G, SafeReach(\lnot S^{ag}_{err} \land \lnot S^{env}_{err}. R'_{\varphi}))$.

\begin{theorem}
Let $\D$ be a planning domain and $\varphi$ an  \LTLf goal in $\D$. Then, $\varphi$ has a cooperative solution in $\D$ iff there exists a cooperatively winning strategy for $(\G, \safereach(\lnot S^{ag}_{err} \cap \lnot S^{env}_{err}, R'_\varphi))$.
% Let $\D$ be a planning domain and $\varphi$ an \LTLf goal on $\D$. Then, an agent strategy $\sigma$ cooperatively realizes $\varphi$ on $\D$ iff it is a cooperatively winning strategy for $(\G, SafeReach(\lnot S^{ag}_{err} \land \lnot S^{env}_{err}, \F'_\varphi))$.
\end{theorem}

% To satisfy this condition we can solve the game \(CoSafeReach(\neg S^{ag}_{err} \land \neg S^{env}_{err}, F_{\varphi})\). 
Here, we reduce to a \DFA game with a pure reachability condition, considering the environment being cooperative:
% However, satisfying this condition is also reducible to solving \textit{cooperatively} reachability game, in which the agent must satisfy the following condition with the environment reacting cooperatively:
% $$
% \Diamond(\neg S^{ag}_{err} \land \neg S^{env}_{err} \land R'_{\varphi}).
% $$

{\centerline{$
\Diamond(\neg S^{ag}_{err} \land \neg S^{env}_{err} \land R'_{\varphi}).
$}}


In our setting, we can solve the reachability game  \((\G, \reach(\neg S^{ag}_{err} \cap \neg S^{env}_{err} \cap R'_{\varphi}))\), considering the environment being cooperative, as listed in step 4 of Algorithm 1.

The following theorem shows that the strategy returned by step 5 of Algorithm 1 satisfies the Criterion of Maximality, thus confirming the correctness of Algorithm 1.
\begin{theorem}\label{thm:correct}
Let $\sigma$ be the strategy returned by Algorithm 1.  For every $h \in \H_\D(\sigma)$ it holds $val(\sigma, h) = val(h)$, hence $\sigma$ is a best-effort strategy.
\end{theorem}
In order to prove Theorem~\ref{thm:correct}, note that the strategy $\sigma$ returned by Algorithm 1 is legal and satisfies the following property: state sequences of $\G$ leading to $W_{adv}$ correspond to histories of the planning domain $\D$, from which the agent can realize $\varphi$ using $\sigma$; state sequences leading to $W_{coop}\backslash W_{adv}$ correspond to histories, from which the agent can cooperatively realize $\varphi$ using $\sigma$; all other state sequences correspond to histories, from which $\varphi$ is unrealizable. The legality of $\sigma$ follows from having the agent perform only legal actions until realizing the goal (if possible) and when the goal is either realized or unrealizable. 
% The legality of $\sigma$ follows from having the agent perform only legal actions until realizing the goal and $nop$ when the goal is realized or unrealizable.
% 
Moreover, we can determine whether a best-effort strategy is winning, pending, or losing by evaluating $val(\sigma, s_0)$. This can be done by checking if the initial state of $\G$ is in $W_{adv}$, $W_{coop} \backslash W_{adv}$, or neither.

We now show the complexity results of \LTLf best-effort synthesis in nondeterministic planning domains.

\begin{theorem}~\label{thm:complexity}
% Best-effort planning for \LTLf goals is:
\LTLf best-effort synthesis in nondeterministic planning domains is:
\begin{compactitem}
    \item 2EXPTIME-complete in the size of the \LTLf goal.
    \item EXPTIME-complete in the size of the domain;
\end{compactitem}
\end{theorem}

Intuitively, the proofs for the lower and upper bounds are based on a reduction from \LTLf FOND planning and the complexity of Algorithm 1, respectively.

% Specifically, we define the  for reachability goals as a pair $\P = (\D, R)$, where $\D$ is  
